Mechanical Search on Shelves with Efficient Stacking and Destacking of Objects

Stacking increases storage efficiency in shelves, but the lack of visibility and accessibility makes the mechanical search problem of revealing and extracting target objects difficult for robots. In this paper, we extend the lateral-access mechanical search problem to shelves with stacked items and introduce two novel policies -- Distribution Area Reduction for Stacked Scenes (DARSS) and Monte Carlo Tree Search for Stacked Scenes (MCTSSS) -- that use destacking and restacking actions. MCTSSS improves on prior lookahead policies by considering future states after each potential action. Experiments in 1200 simulated and 18 physical trials with a Fetch robot equipped with a blade and suction cup suggest that destacking and restacking actions can reveal the target object with 82--100% success in simulation and 66--100% in physical experiments, and are critical for searching densely packed shelves. In the simulation experiments, both policies outperform a baseline and achieve similar success rates but take more steps compared with an oracle policy that has full state information. In simulation and physical experiments, DARSS outperforms MCTSSS in median number of steps to reveal the target, but MCTSSS has a higher success rate in physical experiments, suggesting robustness to perception noise. See https://sites.google.com/berkeley.edu/stax-ray for supplementary material.

==> figures/darss_vs_mctsss.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{dar_mcts_diff_v3.png}
    \caption{Action differences in (A) DARSS and (B) MCTSSS on the same simulated shelf environment. 
    Although the 1D target occupancy distribution appears very similar in the first step, DARSS first explores the largest peak in the occupancy distribution, splitting it into two parts while MCTSSS (rearrangement action) instead chooses to \textit{remove} one of the peaks in the occupancy distribution. Although DARSS reveals a partial view of the target on step 11, it is unable to solve this scene due to \emph{multi-blockage}; the greedy policy is unable to displace the front-most objects blocking the action with the object of the highest support. The policy then takes actions based on the noise in the distribution. On the other hand, MCTSSS benefits from lookahead and reveals the target object.}
    \label{fig:diff_mcts_dar_ss}
    \vspace{-20pt}
\end{figure*}

==> figures/sim_splash.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{figures/sim_splash.png}
    \caption{
    A 16-object scene that requires both restacking and destacking objects to reveal the target object. We compute a pixelwise distribution over likely target object locations, which is overlaid in green and the actions taken by the policy are denoted by red arrows. Since there is not space for rearrangement without blocking grasps on other objects, our policy both reduces the target object occupancy distribution and clears space by restacking the blue cylinder (top left) and destacking the gray box (top right) to allow the pink box to be pushed (bottom left), thus revealing the target object (bottom right). \noteby{AA}{Visually curvy arrows or slanted arrows might help. For example, with the blue block, it would be nice to see that it is taken from the first ``floor'' and put on the second ``floor.''} \todo{replace with real images?}}
    \label{fig:simsplash}
\end{figure}

==> tables/SimRes_old.tex <==

% \begin{table*}[ht]
%     \centering
%     \begin{tabular}{@{}ccccc@{}}\toprule
% No. & Metric & \algabbr & MCTSSS (2, 500) & Oracle \\
% % ======================= No. 6 =========================
% \midrule \multirow{2}*{6}
%   & \SR & \sr{ \textbf{99}}             & \sr{\textbf{99}}       & \sr{99}\\
%   & \SM & \sm{\textbf{2.41}}{1.31}       & \sm{2.53}{1.53}       & \sm{1.67}{0.90}\\
%   & \SA & \sa{\textbf{2.00}}{1.00}{3.00} & \sa{2.00}{1.00}{3.00} & \sa{1.00}{1.00}{2.00}\\
%   & \rt & 19.30s & 114.17s & 65.23s\\
% % ======================= No. 8 =========================
% \midrule \multirow{2}*{8}
%   & \SR & \sr{ \textbf{100}}             & \sr{99}               & \sr{97}\\
%   & \SM & \sm{\textbf{3.27}}{1.97}       & \sm{3.38}{2.24}       & \sm{1.79}{0.85}\\
%   & \SA & \sa{\textbf{3.00}}{2.00}{4.00} & \sa{3.00}{2.00}{4.00} & \sa{2.00}{1.00}{2.00}\\
%  & \rt & 26.25s & 165.25s & 99.98s\\
% % ======================= No.10 =========================
% \midrule \multirow{2}*{10}
%   & \SR & \sr{ \textbf{100} }             & \sr{99}              & \sr{95}\\
%   & \SM & \sm{\textbf{4.23} }{2.81}       & \sm{5.05}{3.67}      & \sm{1.99}{1.21} \\
%   & \SA & \sa{\textbf{4.00}}{2.00}{6.00} & \sa{4.00}{2.00}{7.00} & \sa{2.00}{1.00}{2.00}\\
%   & \rt & 34.92s & 257.24s & 100.35s\\
% % ======================= No.12 =========================
% \midrule \multirow{2}*{12}
%   & \SR & \sr{  98}             & \sr{\textbf{100}}               & \sr{87}\\
%   & \SM & \sm{\textbf{4.26}}{2.67}       & \sm{5.31}{3.78}        & \sm{1.91}{1.22}\\
%   & \SA & \sa{ \textbf{4.00}}{2.00}{6.00} & \sa{4.40}{3.00}{7.00} & \sa{2.00}{1.00}{2.00}\\
%      & \rt & 40.64s & 330.61s & 140.79s\\
% % ======================= No.14 =========================
% \midrule \multirow{2}*{14}
%   & \SR & \sr{  91}             & \sr{\textbf{ 94}}               & \sr{73}\\
%   & \SM & \sm{\textbf{5.57}}{5.04}       & \sm{6.46}{5.51}        & \sm{2.66}{1.70}\\
%   & \SA & \sa{\textbf{4.00}}{2.00}{7.00} & \sa{5.00}{2.00}{9.75}  & \sa{2.00}{1.00}{4.00}\\
%       & \rt & 58.00s & 651.06s & 546.12s\\
% % ======================= No.16 =========================
% \midrule \multirow{2}*{16}
%   & \SR & \sr{ \textbf{88} }             & \sr{82}                & \sr{62}\\
%   & \SM & \sm{\textbf{5.57} }{3.74}       & \sm{8.34}{6.75}       & \sm{2.31}{1.21}\\
%   & \SA & \sa{\textbf{4.50} }{3.00}{7.25} & \sa{6.5}{3.0}{10.75}  & \sa{2.00}{1.00}{3.00}\\
%          & \rt & 73.63s & 908.08s & 663.94s\\
% \bottomrule
%     \end{tabular}
%     \caption{Simulated policy rollouts: 100 trials were executed for 6, 8, 10, 12, 14, and 16 occluding objects for DARSS and MCTSS with maximum depth 2 and rollout number 500; in total, 1200 trials. Oracle policy has access to full state information.}
%     \label{tab:results}
% \end{table*}

\begin{table*}[t!]
    \centering
    \begin{tabular}{@{}lcccccccccccc@{}}\toprule
    & \multicolumn{2}{c}{6 objs} & \multicolumn{2}{c}{8 objs} & \multicolumn{2}{c}{10 objs} & \multicolumn{2}{c}{12 objs} & \multicolumn{2}{c}{14 objs} & \multicolumn{2}{c}{16 objs} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13}
 Policy & \SR & \SA & \SR & \SA & \SR & \SA & \SR & \SA & \SR & \SA & \SR & \SA \\

\midrule
Baseline & \sr{83} & \sa{3}{2}{5} & \sr{79} & \sa{4}{2}{7} & \sr{64} & \sa{4}{1}{7.25} & \sr{50} & \sa{4}{2}{10.75} & \sr{41} & \sa{3}{2}{5} & \sr{22} & \sa{3.5}{2}{7} \\

\midrule
  MCTSSS & \srStar{99} & \saStar{2}{1}{3} & \sr{99} & \saStar{3}{2}{4} & \sr{99} & \sa{4}{2}{7} & \srStar{100} & \sa{4.4}{3}{7} & \srStar{94} & \sa{5}{2}{9.75} & \sr{82} & \sa{6.5}{3}{10.75}\\
  \algabbr & \srStar{99} & \saStar{2}{1}{3} & \srStar{100} & \saStar{3}{2}{4} & \srStar{100} & \saStar{4}{2}{6} & \sr{98} & \saStar{4}{2}{6} & \sr{91} & \saStar{4}{2}{7} & \srStar{88} & \saStar{4.5}{3}{7.25} \\
  
\midrule
  Oracle & \sr{100} & \sa{1}{1}{2} & \sr{100} & \sa{1}{1}{2} & \sr{100} & \sa{2}{1}{3} & \sr{100} & \sa{2}{1}{3} & \sr{98} & \sa{2}{1}{3} & \sr{99} & \sa{3}{2}{4}\\

  
\bottomrule
    \end{tabular}
    \caption{DARSS and MCTSSS(2,500) success rate (SR) and steps taken, shown as median (first quartile, third quartile), for 1200 total trials on shelves with 6--16 occluding objects. Both policies have similar success rates across different numbers of occluding objects, but DARSS reveals the target object more quickly in shelves with more occluding objects.}
    \label{tab:results}
\end{table*}


% \begin{table}[ht]
%     \centering
% \begin{tabular}{@{}cccccccccc@{}}
% \toprule
% \multirow{2}{*}{Policy name}
%           & \multicolumn{9}{c}{Number of Occluding Objects} \\
%           & 6   & 8   & 10  & 12  & 14  & 16  & 20  & 25  & 30 \\ \midrule
% Without Stacking & \textbf{100} & 99  & 99  & 97  & 85  & 73  & 46  & 18  &  3 \\
% DARSS      & 99  & \textbf{100} & \textbf{100} & \textbf{98}  & \textbf{91}  & \textbf{88}  & \textbf{66}  & \textbf{34}  & \textbf{12} \\
% \bottomrule
%     \end{tabular}
%     \caption{\textbf{Success rate over 900 total simulated ablations: Stacking action.} We compare the success rate (\%) of \algabbr with its modified version that cannot perform stacking actions, and observe a significant drop ($\geq10\%$) as the number of objects increases beyond 16 objects. Stacking objects in dense shelf scenes is critical to episode success, as it helps clear up the shelf floor for further push, rearrangement, and destack actions.}
%     \label{tab:ablation_restack}
% \end{table}

==> tables/phy_res.tex <==

% physical
% \begin{table}[t!]
%     \centering
%     \begin{tabular}{@{}lcccccc@{}}\toprule
%  & \multicolumn{2}{c}{6 objs} & \multicolumn{2}{c}{10 objs} & \multicolumn{2}{c}{14 objs} \\
%  \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
%  Policy & \SR & Steps & \SR & Steps & \SR & Steps \\
%  \midrule
%  MCTSSS & \srStar{100} & 2, 3, 2 & \srStar{100} & 14, 5, 16 & \srStar{100} & 3, 7, 5 \\
%  \algabbr & \srStar{100} & 4, 2, 2 & \srStar{100} & 8, 3, 6 & \sr{67} & 3, 4, F \\
% \bottomrule
%     \end{tabular}
%     \caption{Physical experiments using a Fetch robot with 3 trials with 6,10,14 objects for DARSS and MCTSSS(2,500). Showing number of steps to find the target object for each experiment and `F' means the policy fails to find the object in 20 steps.}
%     \label{tab:phy}
%     \vspace{-25pt}
% \end{table}

\begin{table}[t!]
    \centering
    \begin{tabular}{@{}lcccc@{}}\toprule
  Policy & Metric & 6 objs & 10 objs & 14 objs \\
 \midrule
 \multirow{2}{*}{MCTSSS} & \SR& \srStar{100} & \srStar{100} & \srStar{100} \\
 &Steps & 2, 3, 2 & 14, 5, 16  & 3, 7, 5 \\
 
  \multirow{2}{*}{\algabbr} & \SR& \srStar{100} & \srStar{100} & \sr{67} \\
 &Steps & 4, 2, 2 & 8, 3, 6  & 3, 4, F \\

\bottomrule
    \end{tabular}
    \caption{Physical experiments using a Fetch robot with 3 trials with 6,10,14 objects for DARSS and MCTSSS(2,500). Showing number of steps to find the target object for each experiment and `F' means the policy fails to find the object in 20 steps.}
    \label{tab:phy}
    \vspace{-25pt}
\end{table}

==> tables/results.tex <==
% % Define shared row headers
% \newcommand{\SR}{Success Rate}
% \newcommand{\SA}{Median Steps (IQR)}
% \newcommand{\SM}{Mean Steps}

% % Define single format for Success Rate
% % The starred version highlights it
% \newcommand{\sr}[1]{\ifthenelse{\equal{#1}{*}}{\srStar}{\srNoStar{#1}}}
% \newcommand{\srStar}[1]{\textbf{\srNoStar{#1}}}
% \newcommand{\srNoStar}[1]{#1\,\%}

% % Define single format for Step Average + Std
% % The starred version highlights it
% \newcommand{\sa}[1]{\ifthenelse{\equal{#1}{*}}{\saStar}{\saNoStar{#1}}}
% \newcommand{\saStar}[3]{\textbf{\saNoStar{#1}{#2}{#3}}}
% \newcommand{\saNoStar}[3]{#1 (#2 -- #3)}

% % someone pls fix this :( 
% % \newcommand{\sm}[1]{\ifthenelse{\equal{#1}{*}}{\smStar}{\smNoStar{#1}}}
% % \newcommand{\smStar}[2]{\textbf{\smNoStar{#1}{#2}}
% \newcommand{\sm}[2]{#1 $\pm$ #2}






% \begin{table*}[t]
% \vspace{4pt}
% \centering
% % BEFORE MAKING THIS UGLY WITH vertical lines aka "|" PLEASE READ:
% % https://nhigham.com/2019/11/19/better-latex-tables-with-booktabs/
% \begin{tabular}{@{}ccccc@{}}\toprule
% & & 
%     % \multicolumn{2}{c}{\citet{huang2020mechanical}} &
%     \citet{huang2022mechanical} &
%     \multicolumn{2}{c}{S}\\
% \cmidrule(lr){3-4} \cmidrule(lr){5-5} \cmidrule(l){6-7} 
% No. & Metric & DAR & DER-3 & Blulction-DAR & \algabbr & MCTSSS  \\
% \cmidrule{1-7}
% \multirow{2}*{6} % ======================= No. 6 =========================
%   & \SR & \sr{100}   & \sr{100} & \sr{68}         & \sr{72}        & \sr*{92}       \\
%   & \SA & \sa{3.0}{2.0}{3.0} & \sa{2.0}{2.0}{3.0} & \sa{3.0}{1.8}{5.0} & \sa{3.0}{1.0}{4.3} & \sa{2.0}{2.0}{4.0}\\
% \cmidrule{1-7}
% \multirow{2}*{8} % ======================= No. 8 =========================
%   & \SR & \sr{99}  & \sr{100} & \sr{45}         & \sr{50}         & \sr*{88}  \\
%   & \SA & \sa{3.0}{2.0}{4.0} & \sa{2.5}{2.0}{3.0} & \sa{3.0}{1.0}{4.0} & \sa{3.0}{2.0}{4.0} & \sa{3.0}{2.0}{5.0}  \\
% \cmidrule{1-7}
% \multirow{2}*{10} % ======================= No. 10 =========================
%   & \SR & \sr{94} & \sr{100}     & \sr{24} & \sr{34}   & \sr*{67}    \\
%   & \SA & \sa{4.0}{3.0}{6.0} & \sa{3.0}{2.0}{4.0} & \sa{4.5}{2.0}{6.0}  & \sa{3.0}{2.0}{5.0} & \sa{6.0}{3.0}{8.0} \\
% \cmidrule{1-7}
% % \multirow{2}*{12} % ======================= No. 12 =========================
% %   & \SR & \sr{47} & \sr{28}   & \sr{46}   & \sr{}   & \sr{80} & \sr{}     \\
% %   & \SA & \sa{}{} & \sa{5.21}{3.04} & \sa{7.54}{4.68} & \sa{}{} & \sa{4.10}{1.73} & \sa{}{} \\
% % \midrule
% \multirow{2}*{All} % ======================= Avg =========================
%   & \SR & \sr{98}     & \sr{100}   & \sr{54}   & \sr{60}   & \sr*{86}     \\
%   & \SA & \sa{3.0}{2.0}{4.0} & \sa{2.0}{1.0}{3.0} & \sa{2.0}{1.0}{4.0} & \sa{3.0}{1.0}{4.0} & \sa{3.0}{2.0}{4.0} \\
% \bottomrule
% \end{tabular}
% \caption{Simulated policy rollouts: 100 trials were executed for 6, 8, 10, 12, 14, and 16 occluding objects; in total, 3000 trials. For each, we show the \textbf{Success Rate} followed by the \textbf{Median} and \textbf{Interquartile Range (IQR)} for the number of steps taken to reveal the target. Results suggest that suction actions allow the Bluction-DAR policy to succeed between $13\%$ and $38\%$ more often in densely cluttered environments than the best-performing pushing baselines. \todo[inline]{note if stack or not; this is w/o stacks. not sure if we have exp results for bluction-dar for no-stack scenes right now}}
% \label{tab:results}
% \end{table*}

% \begin{table*}[t]
% \vspace{4pt}
% \centering
% % BEFORE MAKING THIS UGLY WITH vertical lines aka "|" PLEASE READ:
% % https://nhigham.com/2019/11/19/better-latex-tables-with-booktabs/
% \begin{tabular}{@{}ccccccc@{}}\toprule
% & & 
%     \multicolumn{2}{c}{Oracle}  &
%     \multicolumn{2}{c}{\citet{huang2020mechanical}} &
%     Bluction \\
% \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(l){7-7} 
% No. & Metric & Oracle-P & Oracle-P+S & DAR & DER-3 & Bluction-DAR   \\
% \midrule
% \multirow{2}*{6} % ======================= No. 6 =========================
%   & \SR & \sr{100}   & \sr{100} & \sr{68}         & \sr{72}        & \sr*{92}       \\
%   & \SA & \sa{3.0}{2.0}{3.0} & \sa{2.0}{2.0}{3.0} & \sa{3.0}{1.8}{5.0} & \sa{3.0}{1.0}{4.3} & \sa{2.0}{2.0}{4.0}\\
% \cmidrule{1-7}
% \multirow{2}*{8} % ======================= No. 8 =========================
%   & \SR & \sr{99}  & \sr{100} & \sr{45}         & \sr{50}         & \sr*{88}  \\
%   & \SA & \sa{3.0}{2.0}{4.0} & \sa{2.5}{2.0}{3.0} & \sa{3.0}{1.0}{4.0} & \sa{3.0}{2.0}{4.0} & \sa{3.0}{2.0}{5.0}  \\
% \cmidrule{1-7}
% \multirow{2}*{10} % ======================= No. 10 =========================
%   & \SR & \sr{94} & \sr{100}     & \sr{24} & \sr{34}   & \sr*{67}    \\
%   & \SA & \sa{4.0}{3.0}{6.0} & \sa{3.0}{2.0}{4.0} & \sa{4.5}{2.0}{6.0}  & \sa{3.0}{2.0}{5.0} & \sa{6.0}{3.0}{8.0} \\
% \cmidrule{1-7}
% \multirow{2}*{12} % ======================= No. 12 =========================
%   & \SR & \sr{94} & \sr{100}     & \sr{24} & \sr{34}   & \sr*{67}    \\
%   & \SA & \sa{4.0}{3.0}{6.0} & \sa{3.0}{2.0}{4.0} & \sa{4.5}{2.0}{6.0}  & \sa{3.0}{2.0}{5.0} & \sa{6.0}{3.0}{8.0} \\
% \midrule
% \multirow{2}*{All} % ======================= Avg =========================
%   & \SR & \sr{98}     & \sr{100}   & \sr{54}   & \sr{60}   & \sr*{86}     \\
%   & \SA & \sa{3.0}{2.0}{4.0} & \sa{2.0}{1.0}{3.0} & \sa{2.0}{1.0}{4.0} & \sa{3.0}{1.0}{4.0} & \sa{3.0}{2.0}{4.0} \\
% \bottomrule
% \end{tabular}
% \caption{Ablation 1: Remove destack in stacked environments}
% \label{tab:ablation_destacking}
% \end{table*}

